Horn Clauses for Communicating Timed Systems

Languages based on the theory of timed automata are a well established approach for modelling and analysing real-time systems, with many applications both in industrial and academic context. Model checking for timed automata has been studied extensively during the last two decades; however, even now industrial-grade model checkers are available only for few timed automata dialects (in particular Uppaal timed automata), exhibit limited scalability for systems with large discrete state space, or cannot handle parametrised systems. We explore the use of Horn constraints and off-the-shelf model checkers for analysis of networks of timed automata. The resulting analysis method is fully symbolic and applicable to systems with large or infinite discrete state space, and can be extended to include various language features, for instance Uppaal-style communication/broadcast channels and BIP-style interactions, and systems with infinite parallelism. Experiments demonstrate the feasibility of the method.

==> eptcsdata.tex <==
\providecommand{\firstpage}{39}
\providecommand{\publicationstatus}{Nikolaj Bj{\o}rner, Fabio Fioravanti, Andrey Rybalchenko, \\ Valerio Senni (Eds.): First Workshop on \\ Horn Clauses for Verification and Synthesis (HCVS 2014)\\
EPTCS 169, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.169.6}{10.4204/EPTCS.169.6}}
\pdfoutput=1

